Efficient Trainable Front-Ends for Neural Speech Enhancement

Many neural speech enhancement and source separation systems operate in the time-frequency domain. Such models often benefit from making their Short-Time Fourier Transform (STFT) front-ends trainable. In current literature, these are implemented as large Discrete Fourier Transform matrices; which are prohibitively inefficient for low-compute systems. We present an efficient, trainable front-end based on the butterfly mechanism to compute the Fast Fourier Transform, and show its accuracy and efficiency benefits for low-compute neural speech enhancement models. We also explore the effects of making the STFT window trainable.

==> old_sections/fft_arch_old.tex <==
\section{The FFT as a Network Layer}
Consider the typical matrix FFT derivation for a 4 point FFT. Intuitively, the FFT factors the DFT matrix into a set of sparse matrices. FFT algorithms leverage this highly structured sparsity for speed. We will leverage this sparsity for both speed and storage.

\[\textit{FFT}(X) = W_1 W_0 X\]
\[\textit{FFT}(X) =
\begin{bmatrix}
    1  & 0    & W_4^0    & 0 \\
    0  & 1    & 0    & W_4^1 \\
    1  & 0    & -W_4^0    & 0 \\
    0  & 1    & 0    & -W_4^1
\end{bmatrix}
\begin{bmatrix}
    1  & 1    & 0    & 0 \\
    1  & -1    & 0    & 0 \\
    0  & 0    & 1    & 1 \\
    0  & 0    & 1    & -1
\end{bmatrix}
X\]

Note that the matrices are block diagonal or composed of stacks of diagonal matrices. This will hold for the general $N$ point FFT which can be expressed as a set of $\log_2(N)+1$ sparse matrix multiplies. \ref{fig:fft_sketch} visualizes these matrices and the associated sparsity pattern.
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.8]{figures/fft_factor_trace.pdf}
    \caption{This matrix product demonstrates how to implement the FFT in a trainable setup. Each step of the FFT can be represented by a sparse matrix. The matrices are highly structured which acts as a kind of regularization. }
    \label{fig:fft_sketch}
\end{figure}

Rigorously, in general, the $N$ point FFT can be expressed using an $N$ point bit reversal permutation matrix $P_N$, identity matrices $I$, matrices with complex exponential down the diagonal $\Omega$, and the Kronecker product $\otimes$

Define the $N$ point FFT as $F_{N} =A_{t} \cdots A_{1} P_{N}$ where $t = \log_2(n)$. We will use the dummy variables $L = 2^q, r= \frac{n}{L}$ such that $\Omega_{\frac{L}{2}} = \operatorname{diag} \left(1, \omega_{L}, \ldots, \omega_{L}^{\frac{L}{2}-1}\right)$ and $\omega_{L}= e^{\frac{-2 \pi j}{L}}$

Finally, for each $A$ in $F_{N}$:
\begin{equation}
    A_{q} =I_{r} \otimes \left[
    \begin{array}{cc}
        I_{L / 2} &  \Omega_{L / 2} \\ 
        I_{L / 2} & -\Omega_{L / 2}
    \end{array} \right]\\
\end{equation}


\subsection{Forwards FFT}
This set of matrix multiplies can be represented as a neural network with several sparsely connected layers. The DFT on the other hand is a single layer with dense connectivity. We preserve the general FFT structure by only connecting network nodes on the block diagonal structure given by the FFT. This preserves the speed and structure of the FFT while both reducing the number of parameters in the front-end and operating on the raw waveform. The figure below illustrates the DFT and FFT connectivity structures and how they may be interpreted as neural network layers.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.71]{figures/butterfly_structure_4.pdf}
    \caption{On the left we show the connectivity pattern enforced by a DFT matrix. It is simply a fully connected layer since the DFT matrix application can be represented by a matrix multiply. On the right we show the connectivity pattern enforced by the FFT algorithm. This connectivity plot is very sparse and requires far fewer calculations than the DFT matrix.}
    \label{fig:butterfly}
\end{figure}

Finally, throughout these transforms we explicitly model the real and imaginary components. When initialized correctly, these models return identical results to the FFT algorithm.


\subsection{Backwards FFT}
To compute the inverse FFT we use the simple conjugate trick. Given some Fourier transform $X[k]$ of the time series $x[n]$. It is possible to compute the inverse Fourier transform of $X[k]$ using only the forward FFT. In particular: 
\[x=\frac{\overline{\textit{FFT}(\overline{X(\omega)})}}{N}\].

In our model we leverage this property. However, the forward FFT layer and the inverse FFT layer do not share parameters. We use different learned FFTs for the forward and inverse transforms. These FFT layers are initialized and updated as separate entities.

%\shri{This part is unclear too...perhaps needs a bit more explanation}
% & L = 2^q, r= \frac{n}{L} \\
% \Omega_{\frac{L}{2}} &= \operatorname{diag} \left(1, \omega_{L}, \ldots, \omega_{L}^{\frac{L}{2}-1}\right), \omega_{L}= e^{\frac{-2 \pi j}{L}} \\
% https://www.cs.cornell.edu/~bindel/class/cs5220-s10/slides/FFT.pdf
% slide 17 from these slides -- this may make sense to pose it as just an entire set of aprase dense layers.
% \shri{This threw me off. I think there should be some more explanation here. I think a good strategy of explaining math heavy stuff would be to first give the bigger picture first, then try to intuitively develop the equation. So, I'd start off with saying that FFT tries to reduce the complexity by computing the Fourier transform as product of sparse matrices. What you have after the equations should probably go before.}


% Given the constraints of low compute and small memory we want to leverage the fast fourier algorithm in tandem with state of the art end-to-end systems. We do this by expressing the N point FFT in a learnable and differentiable format. In particular, we adopt the tukey-cooley sparse matrix factorization. This factorization says that for an $n$ point DFT $F_n$ with a $t = \log_2(n)$ and bit reversal permutation matrix $P_n$:

% This definition expresses the FFT as product of sparse matrices. Matrix multiplies fit naturally in the deep learning framework meaning that we can construct network layers which mimic this sparse structure.


% Viewing the traditional learned front-ends as windowing operations followed by dense $\mathbf{O}(n^2)$ matrix multiplies we can incorporate the FFT into a neural network and vastly reducing compute requirements. The below figure shows a learned front-end with a dense layer and a learned front-end with sparse FFT layers side-by-side. Note that the FFT setup is just the classic decimation in time butterfly structure. 



% Note that the FFT is a many layered transform with fewer parameters per layer. Usually with DNNs models with more layers and fewer parameters per layer perform better than shallow models with very wide layers.

% The butterfly diagram can be though of as a sequence of highly restricted linear layers where the weight matrices are sparse and block diagonal. This is also similar to a set of dilated convolutions. For example, the factorization for a 4 point FFT yields:

% Where $W_i$ is the structure for the $i^{th}$ layer and $X$ is the input data vector after bit reversal.


% The first layer is a block diagonal matrix where the diagonal is made up of $2 \times 2$ dfts. The $n^{th}$ layers are then made up of only twiddle factors and only have values on the main diagonal and on some $k^{th}$ super and sub diagonals.

% More intuitively, the matrix sketch for factoring would be like this:

==> old_sections/intro_old.tex <==
\section{Introduction}
Neural network based techniques have vastly improved speech enhancement and source separation performance \cite{venkataramani2018end, luo2018tasnet, luo2019conv, shi2019deep, rethage2018wavenet}. Recent advances include models which can separate arbitrary numbesr of speakers \cite{hershey2016deep}, adaptations of generative adversarial networks to audio \cite{pascual2017segan}, and numerous U-Net \cite{ronneberger2015u} based systems \cite{ macartney2018improved, stoller2018wave}.  These methods rely on very deep networks with potentially millions of parameters. Operating directly on the waveform has proven very beneficial for some models \cite{venkataramani2018end, luo2018tasnet, luo2019conv, shi2019deep, stoller2018wave, rethage2018wavenet}. These models are based on learning transforms optimized for the task at hand. In essence, they contain STFTs with trainable parameters. 

As such, neural speech enhancement with a trainable STFT has become a powerful tool for high performance models. The first layer(front-end) of these neural models performs windowing followed by a dense matrix multiply. Trainable STFT models allow this dense matrix to be updated; fixed STFT models leave it as the DFT matrix. Initial work on learning this matrix focused on reconciling the issues of real valued square transforms as a front-end \cite{venkataramani2018end}. Future work focused on more powerful masking networks for learned transforms, examining recurrent systems \cite{luo2018tasnet}, and fully convolutional systems \cite{luo2019conv}. They also found that using a rectangular over-complete front-end worked well. Most recently \cite{shi2019deep} used dilated convolutions in the masking network achieving current state of the art in source separation. Note that these model all also learn a back-end which inverts the front-end via another dense matrix multiply and the overlap-add method.

Low compute acoustic scenarios are on the rise in the form of hearables which involve wearable audio devices. These devices come with stringent compute requirements but offer the opportunity for audio processing everywhere. In these contexts, storing and performing inference with the dense matrix inside a trainable STFT is an expensive task. To learn an STFT with $512$ point transforms takes $2 \times 512 \times 512 = 524288$ parameters. Running this system on an embedded or low compute device would be cumbersome. The front-end parameters alone would fill a modern processors L2 cache. This leaves no room for the rest of the model. We aim to address this issue by creating an efficient front-end for models operating on the waveform.

In this work we propose an efficient learned front-end which we use for speech enhancement. Our front-end is inspired by the FFT and when correctly initialized still computes the FFT in $\mathbf{O}(n \log n)$ time. We evaluate this model on the VCTK speech enhancement task \cite{valentini2017noisy} and show that this front-end outperforms fixed front-ends despite no increase in compute and minimal increase in the number of required parameters. Additionally, we propose to learn a window. In the case of learning an STFT the trainable dense matrix can have a window pre-applied to it's rows. However, since our model learns an algorithm to compute representation with respect too some basis and not an explicit basis we include a separate windowing operation. In the spirit of real-time enhancement our model is also entirely causal.

% \shri{I think the focus of this introduction is a little too much on Adaptive front ends and very less on low compute situations. I would write this intro as an extension of the abstract itself where you explain the abstract in a bit more detail with some supporting references. So, in the intro, I would say something along the lines of .... with deep learning and neural networks there has been a solid improvement in source separation performance. (some references for this). Operating direcly on the waveforms has proven very beneficial (refs for this)... Then a bit of idea on how people design adaptive front ends... Then why is this a problem on low compute situations... the front end can have more parameters than the separation network itself.... some number here would help a lot. Ritwik should know this. Then talk about what we propose and how we solve the problem... I think you have most of the stuff in there already, just a bit shuffling around required.}


% I really don't like my pitch
% Maybe we should come with a different perspective

% We could pitch this as another way to do end-to-end training for small models 
% and that we demo this on speech enhancement.

% We shouldn't pitch this as an FFT alternative. Instead, pitch from the perspective of high resource constraints.

% Other recent advances in speech separation and enhancement include adaptation of the U-Net architecture \cite{ronneberger2015u} to speech systems \cite{macartney2018improved, stoller2018wave, ronneberger2015u, rethage2018wavenet} and the use of generative adversarial networks \cite{pascual2017segan}.


%\cite{luo2018tasnet, luo2019conv} some properties of this layer are explored and it is found that the model learns a filter-bank with a logarithmic frequency responses distribution. While these masking based learned transform methods have strong performance they require learning a large first layer. In \cite{venkataramani2018end} an $N$ point DFT matrix sized kernel is learned meaning the first layer requires $N^2$ parameters. In \cite{luo2018tasnet, luo2019conv} an overcomplete basis is learned of size $N \times k$. In both cases, even the front-end transform would take up almost all of  the L2 cache on a cpu.


% Neural networks methods have become the tool of choice for speech enhancement and source separation tasks. These methods generally fall into two categories: masking based and non-masking. The non-masking models such as those proposed in  \cite{rethage2018wavenet} operate on raw waveforms and never explicitly produce a mask which is applied to the input. Some more recent work from the medical segmentation community proposes the use of a U-net architecture \cite{ronneberger2015u}. This lead to \cite{macartney2018improved, stoller2018wave} which have no explicit masking step but do have numerous residual connections. Most models that are masking based have an explicit latent representation of the signal in the learned transform domain. These models include \cite{venkataramani2018end, luo2018tasnet, luo2019conv} which all explicitly produce a mask that is applied to some transformed input. 


